First studies on cascaded dual-phase liquid hole-multipliers in xenon

Challenges in scaling up noble-liquid time projection chambers prompted the exploration of new detection concepts. The liquid hole-multiplier (LHM) was introduced as a potential component, enabling the detection of ionization electrons and VUV photons. Prior studies focused on perforated electrodes coated with CsI immersed in the liquid and electroluminescence amplification produced on a bubble trapped underneath. However, the performance was hindered by electron transfer across the liquid-gas interface. Here, we explored a bubble-free variant, placing a CsI-coated Thick Gas Electron Multiplier electrode below the liquid-gas interface to improve the transfer efficiency across it. Results show >5-fold improvement in the S1'/S2 ratio (a proxy for the photon detection efficiency (PDE)) compared to the bubble-assisted LHM. Although the achieved PDE is still below expectation ($\sim$4%), we propose potential improvements to enhance the performance of this detector.

==> src/leftovers.tex <==
\subsection{Setup for the extraction measurement}

The measurement of the electron extraction into gas phase consists of an alpha source held in a metallic frame and a mesh that are fully immerse in liquid.
In the gas phase we place a THGEM and the interface lies somewhere in between the mesh and the THGEM.
This scheme is depicted in Figure \ref{fig:extraction_setup}.
The mesh above the source that the field across the interface is homogeneous.
Finally, by using a THGEM we are able to apply a reverse field between both sides of the electrode, ensuring that the electrons are not dispersed sideways, as they are focused into the bottom plane.

\begin{figure}
    \centering
    \includegraphics[height=6cm]{img/extraction_setup.png}
    \caption{Schematic diagram of the setup used for the extraction efficiency measurement.}
    \label{fig:extraction_setup}
\end{figure}


==> src/tiling.tex <==
\section{Large-area THGEM electrodes}
\label{sec:tiling}

The maximum size of THGEM electrodes that can be currently produced is $\sim$0.2-0.25~m$^2$ \cite{AGARWALA2020161832, BRESSLER2020162861, Song_2020}.
However, future DM detectors, with active masses of $\sim$50 tonnes, are planned as cylindrical TPCs exceeding 2~m in diameter  \cite{Aalbers_2016, Aalseth_2018}.
These detectors would require tiling the detector with THGEM electrodes and devising an efficient support structure with minimal dead areas.
%Therefore, in order to build a TPC with these dimensions, it is necessary to tile THGEM electrodes.
%This requires a support structure that generates dead areas, which can compromise the performance of the detector due to electron loss at the THGEM boundaries.

This can be avoided by introducing an electrode (e.g. a conductive strip or wire) in the support structure that diverts electrons towards the active area of the surrounding electrodes.
We performed finite element calculations in COMSOL Multiphysics\registered to validate this hypothesis.
Figure \ref{fig:tiling} shows the field lines for the junction of two THGEM electrodes with similar parameters to the ones used in our experiments without (left panel) and with (right panel) a conductive strip within the support structure.
The frame supporting the L- and G-THGEM, made of an insulating material, are 5~mm wide and 5~mm thick.
The conductive strip is 1~mm-wide and the two THGEM electrodes are separated by a 6~mm gap.
For a drift field of 800 V/cm a voltage difference between the bottom face of the L-THGEM and the strip of 1400 V is sufficient to redirect the field lines towards the active area.

We observe that, without the strip, there is a significant fraction of field lines going through the support structure, which can be translated into electron loss at the boundary.
However, the field configuration with the strip prevents these losses by redirecting the field lines towards the active area of the THGEM.

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{img/tiling.png}
    \caption{COMSOL calculation of the tiling of two large-area THGEMs without (left) and with (right) a conductive strip to avoid electron loss at the boundaries. See text for details.}
    \label{fig:tiling}
\end{figure}
